Massive Neutrinos: Phenomenological and Cosmological Consequences

In this thesis we will address three different phenomena related to neutrino physics: mass models, detection of the cosmic neutrino background and the neutrino background in Dark Matter searches, considering the different characteristics in each case. In the study of neutrino mass models, we will consider models for both Majorana and Dirac neutrinos; specifically, we will probe the neutrinophilic two-Higgs-doublet model. Regarding the detection of relic neutrinos, we will analyse the consequences of the existence of physics beyond the Standard Model in the capture rate by tritium. Finally, we will scrutinize the impact of neutrinos in Direct Detection searches of Weakly Interacting Massive Particles (WIMP) including Standard Model plus additional interactions in the form of simplified models.

==> Preambulo/Dedicatoria.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEDICATORIA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{10cm}
\thispagestyle{empty}

\begin{flushright}
	{\calligra\Large
		Hola mundo!
	}
\end{flushright}

